Selecting time-series hyperparameters with the artificial jackknife

This article proposes a generalisation of the delete-$d$ jackknife to solve hyperparameter selection problems for time series. I call it artificial delete-$d$ jackknife to stress that this approach substitutes the classic removal step with a fictitious deletion, wherein observed datapoints are replaced with artificial missing values. This procedure keeps the data order intact and allows plain compatibility with time series. This manuscript justifies the use of this approach asymptotically and shows its finite-sample advantages through simulation studies. Besides, this article describes its real-world advantages by regulating forecasting models for foreign exchange rates.

==> ch1_annex/subsect1.tex <==

\clearpage

\begin{definition}[Categories of forecasts]\label{ch1:def:forecasttype}
	To emphasise this point, denote $\vect{\hat{Y}}_{t+1|s}(\vect{\gamma})$ as
	\begin{align*}
		\begin{cases}
			\text{in-sample}, &\text{ if } t+1 \leq \max \blpar \mathscr{I}(s) \brpar, \\
			\text{pseudo out-of-sample}, &\text{ if } \max \blpar \mathscr{I}(s) \brpar < t+1 \leq T, \\
			\text{out-of-sample}, &\text{ if } t+1 > T,
		\end{cases}
	\end{align*}
	
	\noindent where $\max \blpar \mathscr{I}(s) \brpar$ is the largest integer in $\mathscr{I}(s)$ and $p \leq t \leq T$.
\end{definition}

\noindent The second and third cases are equally realistic, but target different forecast horizons. Indeed, the third case is the only one targetting a point in time outside the full sample.

For in-sample and pseudo out-of-sample forecasts, this manuscript measures the realised error using the quadratic loss function in \cref{ch1:def:forecasterr}.

Out-of-sample forecasts are particularly interesting for hyperparameter selection, because they are the only ones that can be used in order to formalise the idea of predicting well unseen future datapoints. Despite that, a direct measure of out-of-sample error cannot be computed following the approach in \cref{ch1:def:forecasterr} since future observations are obviously unknown. Therefore, an alternative is needed.








